CapsFake: A Multimodal Capsule Network for Detecting Instruction-Guided Deepfakes

The rapid evolution of deepfake technology, particularly in instruction-guided image editing, threatens the integrity of digital images by enabling subtle, context-aware manipulations. Generated conditionally from real images and textual prompts, these edits are often imperceptible to both humans and existing detection systems, revealing significant limitations in current defenses. We propose a novel multimodal capsule network, CapsFake, designed to detect such deepfake image edits by integrating low-level capsules from visual, textual, and frequency-domain modalities. High-level capsules, predicted through a competitive routing mechanism, dynamically aggregate local features to identify manipulated regions with precision. Evaluated on diverse datasets, including MagicBrush, Unsplash Edits, Open Images Edits, and Multi-turn Edits, CapsFake outperforms state-of-the-art methods by up to 20% in detection accuracy. Ablation studies validate its robustness, achieving detection rates above 94% under natural perturbations and 96% against adversarial attacks, with excellent generalization to unseen editing scenarios. This approach establishes a powerful framework for countering sophisticated image manipulations.

==> Main_expr_Table.tex <==
\begin{table*}[t]
\centering
\caption{Deepfake detection performance across benchmark datasets.}
\begin{tabular}{lcccc}
\hline
\textbf{Dataset} & \textbf{Methods} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Accuracy} \\
\hline
\multirow{6}{*}{MagicBrush} 
& DE-FAKE & 79.81 & 92.34 & 85.62 & 84.49 \\
& ZeroFake & 53.02 & 61.68 & 57.29 & 54.02 \\
& DCT & 98.85 & 96.26 & 97.54 & 97.57 \\
& UnivCLIP & 69.78 & 71.21 & 70.49 & 70.19 \\
& UnivConv2B & \textbf{100.0} & 94.58 & 97.21 & 97.29 \\
& \textbf{CapsFake (Ours)} & 98.71 & \textbf{100.0} & \textbf{99.35} & \textbf{99.35} \\
\hline
\multirow{6}{*}{SEED-Data-Edit-Part1-Unsplash}
& DE-FAKE & 89.53 & 76.93 & 82.75 & 83.97 \\
& ZeroFake & 56.66 & 55.33 & 55.99 & 56.50 \\
& DCT & 88.06 & 71.80 & 79.10 & 81.03 \\
& UnivCLIP & 85.18 & 85.80 & 85.49 & 85.43 \\
& UnivConv2B & 93.98 & 95.80 & 94.88 & 94.83 \\
& \textbf{CapsFake (Ours)} & \textbf{99.20} & \textbf{99.80} & \textbf{99.50} & \textbf{99.50} \\
\hline
\multirow{6}{*}{SEED-Data-Edit-Part1-Openimages}
& DE-FAKE & 72.03 & 46.32 & 56.38 & 64.17 \\
& ZeroFake & 57.53 & 27.11 & 36.85 & 53.55 \\
& DCT & 77.04 & 41.68 & 54.09 & 64.63 \\
& UnivCLIP & 71.75 & 53.93 & 61.58 & 66.35 \\
& UnivConv2B & 63.58 & 77.65 & 69.91 & 66.58 \\
& \textbf{CapsFake (Ours)} & \textbf{88.27} & \textbf{93.79} & \textbf{90.95} & \textbf{90.66} \\
\hline
\multirow{6}{*}{SEED-Data-Edit-Part2-3 (Multi-turn)}
& DE-FAKE & 81.01 & 62.16 & 70.34 & 73.79 \\
& ZeroFake & 56.67 & 38.56 & 45.89 & 54.54 \\
& DCT & 57.23 & 62.93 & 59.94 & 57.95 \\
& UnivCLIP & 77.11 & 65.40 & 70.77 & 72.99 \\
& UnivConv2B & 75.10 & 85.75 & 80.07 & 78.66 \\
& \textbf{CapsFake (Ours)} & \textbf{95.38} & \textbf{90.92} & \textbf{90.92} & \textbf{93.26} \\
\hline
\end{tabular}
\label{tab:benchmark_results}
\end{table*}


==> Table_1.tex <==
\begin{table}[th]

    \begin{centering}
    \caption{Cross-domain transferability analysis: F1 scores (\%) for intra-domain and inter-domain evaluations. $X \rightarrow Y$ represents training on domain $X$ and testing on domain $Y$, where G: GLIDE, V: VQDM}\label{tab:test_transferability}
    %\caption{Transferability performance: F1 score (\%) on seen and unseen Domains. Baseline models demonstrate strong generalization within the same domain but show a marked drop in performance on unseen domains. $X \rightarrow Y$ denotes that the model is trained on domain $X$ and tested on domain $Y$. (G: GLIDE, V: VQDM)}\label{tab:test_transferability}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Methods & G$\rightarrow$G & G$\rightarrow$V & V$\rightarrow$V & V$\rightarrow$G\tabularnewline
    \hline
    DE-FAKE \cite{shaFAKEDetectionAttribution2023} & 98.86 & 34.42 & 95.45 & 51.40 \tabularnewline
    \hline
    UnivCLIP \cite{ojhaUniversalFakeImage2024} & 97.63 & 28.57 & 97.39 & 43.04 \tabularnewline
    \hline
    UnivConv2B \cite{abdullahAnalysisRecentAdvances2024} & 99.97 & 33.17 & 99.76 & 78.70 \tabularnewline
    \hline
    DCT \cite{rickerDetectionDiffusionModel2024} & 99.20 & 45.84 & 97.32 & 64.45 \tabularnewline
    \hline
    \end{tabular}
    \par\end{centering}
  \end{table}

